Source Code Recommender Systems: The Practitioners' Perspective

The automatic generation of source code is one of the long-lasting dreams in software engineering research. Several techniques have been proposed to speed up the writing of new code. For example, code completion techniques can recommend to developers the next few tokens they are likely to type, while retrieval-based approaches can suggest code snippets relevant for the task at hand. Also, deep learning has been used to automatically generate code statements starting from a natural language description. While research in this field is very active, there is no study investigating what the users of code recommender systems (i.e., software practitioners) actually need from these tools. We present a study involving 80 software developers to investigate the characteristics of code recommender systems they consider important. The output of our study is a taxonomy of 70 "requirements" that should be considered when designing code recommender systems. For example, developers would like the recommended code to use the same coding style of the code under development. Also, code recommenders being "aware" of the developers' knowledge (e.g., what are the framework/libraries they already used in the past) and able to customize the recommendations based on this knowledge would be appreciated by practitioners. The taxonomy output of our study points to a wide set of future research directions for code recommenders.

==> tables/design-tables.tex <==
% !TEX root = ../main.tex

% Design tables. 

\begin{table}[ht]
	\centering
	\caption{Number of functions and tokens for all datasets.}
	\scriptsize
	\label{tab:dataset}
	\begin{tabular}{llrr}
	\toprule
	\multirow{2}{*}{\bf Dataset} & \multirow{2}{*}{\bf Split} & \multirow{2}{*}{\bf \#Instances} & \multirow{2}{*}{\bf \#Tokens}\\ 
	& & \\\midrule
		              Pretraining        &   & 1M & 52.9M\\\midrule

	                      &  Training & 1.15M & 74.0M\\
	          Finetuning            &                                Evaluation & 144k & 9.3M\\
	                      &                                Test & 144k & 9.2M\\
	                      \bottomrule
\end{tabular}
\end{table}
	


==> tables/parameters.tex <==
% !TEX root = ../main.tex

% Design tables. 

\begin{table}[ht]
	\centering
	\caption{Parameter used for slanted configuration during finetuning.\vspace{-0.2cm}}
	\scriptsize
	\label{tab:params}
	\begin{tabular}{lr}
	\toprule
	{\bf Parameter}  & {\bf Value}\\\midrule
	Batch size & 256\\
	Training steps & 700k\\
	cut\_fraction & 0.1\\
	ratio & 32\\
	max\_learning\_rate & 0.01\\
	start\_step & 0\\
\bottomrule
\end{tabular} 
% \vspace{-0.5cm}
\end{table}
% \vspace{0.2cm}

